TierBase: A Workload-Driven Cost-Optimized Key-Value Store

In the current era of data-intensive applications, the demand for high-performance, cost-effective storage solutions is paramount. This paper introduces a Space-Performance Cost Model for key-value store, designed to guide cost-effective storage configuration decisions. The model quantifies the trade-offs between performance and storage costs, providing a framework for optimizing resource allocation in large-scale data serving environments. Guided by this cost model, we present TierBase, a distributed key-value store developed by Ant Group that optimizes total cost by strategically synchronizing data between cache and storage tiers, maximizing resource utilization and effectively handling skewed workloads. To enhance cost-efficiency, TierBase incorporates several optimization techniques, including pre-trained data compression, elastic threading mechanisms, and the utilization of persistent memory. We detail TierBase's architecture, key components, and the implementation of cost optimization strategies. Extensive evaluations using both synthetic benchmarks and real-world workloads demonstrate TierBase's superior cost-effectiveness compared to existing solutions. Furthermore, case studies from Ant Group's production environments showcase TierBase's ability to achieve up to 62% cost reduction in primary scenarios, highlighting its practical impact in large-scale online data serving.

==> architecture.tex <==
\vspace{-0.5cm}
\section{Disaggregated Cache-Storage Architecture}
In this section, we introduce the disaggregated cache-storage architecture that deviates from the conventional caching model. Before introducing the details of our proposed architecture, let us first revisit the traditional separated cache and database architecture.

As depicted in Figure  \ref{fig:disk}, the traditional architecture stores primary data within a disk-based database, such as MySQL \cite{mysql} or OceanBase \cite{OB}, and transfers it to a distributed in-memory cache, like Redis cluster, as needed. The workflow of this architecture illustrates the process by which queries from an application are managed. Steps depicted in gray are optional and occur only when the cache is missing. While this approach provides a cost-effective solution for large datasets, it introduces development complexity in maintaining data consistency between the cache and the database.

Figure \ref{fig:inmem} depicts the workflow of an in-memory database with persistence, such as Redis clusters with AOF (Append-Only File) persistence, store all data in memory for fast access and persist the data to disk for durability. Although this approach offers excellent performance, it can be expensive for large datasets, as all data must be stored in memory.

As illustrated in Figure \ref{fig:disa}, the disaggregated cache-storage database diverges from the traditional caching model by mandating that users interact exclusively with the cache tier. This architectural choice significantly simplifies the process of maintaining data consistency between the cache and storage tiers. Moreover, it minimizes network round trips, thereby reducing the overhead typically associated with conventional caching architectures. In contrast to in-memory databases, the disaggregated architecture achieves substantial cost savings by keeping only the frequently accessed (hot) data in the cache (in-memory) tier, while less frequently accessed (cold) data is stored in the more cost-effective storage tier.

Furthermore, we deploy the classic write-through and write-back caching policies into the disaggregated architectures, which introduce unique challenges. In traditional contexts, these policies are implemented within a single tier, where the cache and storage are tightly coupled. In contrast, the separation of cache and storage tiers in a disaggregated architecture introduces new complexities in maintaining data consistency and synchronization. The cache and storage tiers operate independently, communicating over a network, which can introduce latency and potential failures. Ensuring data consistency between the tiers requires careful design that can handle the challenges posed by the disaggregated nature of the architecture. In Section \ref{sec:writethough_back}, we will discuss the design considerations and optimization strategies to handle these challenges.

Please note that each of the architectures illustrated in Figure \ref{fig:arch} has its specific use cases. For example, the architecture shown in Figure \ref{fig:disk} is usually used as a caching system, while the architectures shown in Figures \ref{fig:inmem} and \ref{fig:disa} are used as databases with persistence. We argue that TierBase is designed to support all three use cases through flexible configuration. Such flexibility aids in selecting the most cost-effective settings while fulfilling the application's requirements.

Cache-storage disaggregation differs from other disaggregated architectures. In disaggregated storage like \cite{Aurora,Socrates,PolarDB,tao,Crystal}, compute nodes are stateless and focus on query computation, while storage is separate and shared. Disaggregated memory architectures \cite{Ditto,rdma1,Sherman} aim to extend memory capacity beyond a single server, but require specific hardware, such as RDMA and CXL, alongside rack-scale configurations to ensure low latency. In contrast, cache-storage disaggregation employs a shared-nothing cache service in the cache tier, operating independently from the storage tier. This allows efficient handling of skewed data accesses at a large scale while ensuring data synchronization between cache and storage tiers, without the need for specialized hardware.


==> costmodel.tex <==
\section{Cost Model}\label{sec:cost_model}

In this section, we introduce the cost model proposed and evaluated in  this paper. The cost model simplifies the cost computation of key-value storage based on our analysis of the real system in Ant Group. We ingeniously design the cost model to measure the performance and storage cost in the unified model. %\textbf{TODO add more words for model features}

Please note that our cost model analysis is designed more for scenarios like online services where quick response times are critical. For offline data analysis tasks, which typically process large volumes of data without strict time constraints, the cost considerations may vary significantly.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/cost_model.jpg}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.35]{figures/cost_model1.pdf}
  \caption{Cost model (Performance vs Capacity)}
  \label{fig:cost-model}
  % \vspace{-2mm}
\end{figure}
% \vspace{1pt}
\subsection{Cost Analysis}

\textbf{Performance Cost.}
 In NoSQL databases, performance cost reflects the resource utilization for data read and write operations, including CPU overhead, network I/O, disk IOPS consumption, and memory bandwidth usage. These factors are crucial in determining overall system performance, affecting throughput and latency.
 
%In NoSQL database systems, the performance cost reflects the resource utilization during data storage and retrieval. This includes CPU overhead, representing the computational demands on the CPU; network I/O overhead, denoting the load on network resources; disk IOPS consumption, which measures the rate of input/output operations on storage devices; and memory bandwidth utilization, assessing the usage of the system's memory data transfer capacity. These aspects are crucial in determining the overall system performance, affecting throughput and latency.

%Performance cost in NoSQL database systems refers to the quantitative impact on system resources that result from data storage and retrieval operations. This mainly encompasses:

%CPU Overhead: The computational workload imposed on the CPU due to storage-related tasks, which can detract from its availability for other processing activities. The overhead is often measured as a percentage of CPU cycles consumed by storage operations relative to the total available cycles.

%Network I/O Overhead: This refers to the utilization and operational load imposed on the network infrastructure by storage activities. It can be quantified by the volume of data transmitted over the network, measured in bits per second, and the number of network packets that must be processed by network interfaces. High Network I/O can create bottlenecks, resulting in increased response times and decreased overall network efficiency. It is a critical performance cost metric in environments where data is frequently accessed or transferred over a network, such as in cloud computing and disaggregated storage systems.

%Disk IOPS Consumption: The rate of input/output operations a storage device is performing, which is a critical determinant of its ability to handle read and write requests. Higher IOPS consumption can indicate a greater demand on the storage subsystem and can lead to increased latency if the demand approaches or exceeds the device's performance capabilities.

%Memory Bandwidth Utilization: The proportion of the data transfer capacity of the system's memory interface that is consumed by storage traffic. High memory bandwidth utilization can lead to contention among multiple concurrent processes and impact overall system performance.

%In summary, the performance cost in storage systems is a composite measure that captures the extent to which storage operations consume critical system resources, potentially leading to reduced throughput and increased latency in overall system performance. 
\noindent\textbf{Capacity Cost.}
Capacity cost is influenced by the resources and expenses involved in data storage, varying based on the storage medium and number of replicas. For caching systems and in-memory databases, it is linked to the volume of data in RAM, which offers faster access but at a higher cost. Disk-based storage systems incur costs based on total disk space used, typically providing a more economical solution for larger data volumes. The cost also incorporates considerations for data redundancy, essential for reliability and availability.

%The capacity cost in database systems is influenced by the resources and expenses involved in data storage. This cost varies based on the storage medium and the number of replicas. For caching systems and in-memory databases, it is linked to the volume of data held in RAM, which offers faster access but at a higher cost. In contrast, disk-based storage systems incur costs based on the total disk space used, which typically provides a more economical solution for larger data volumes. The cost also incorporates considerations for data redundancy, essential for ensuring reliability and availability.
%Capacity cost represents the total resources and associated expenses required to store data within a system. This cost is directly influenced by the amount of data that can be accommodated by the storage medium, whether it be memory or disk space, and by the redundancy of the data, as determined by the number of physical replicas maintained for reliability and availability purposes.

%For an in-memory store, the capacity cost is determined by the volume of data that can be held in the system's primary memory (RAM). Since in-memory storage typically provides faster access to data but comes with a higher cost per unit of storage, the capacity cost here is a function of the available RAM, which is more expensive than disk storage.

%For a disk-based storage system, the capacity cost is influenced by the total size of the disk space available for storing data. Disk space tends to be cheaper per unit than RAM, allowing for more data to be stored at a lower cost. % However, the capacity cost also includes the overhead of creating and managing physical replicas of the data. These replicas serve to protect against data loss due to disk failures and contribute to the overall capacity cost due to the additional disk space they require.

%In essence, capacity cost in a storage system is determined by the amount of data a user needs to store and the choices made regarding the storage media and the level of data replication.
\noindent\textbf{Performance Cost v.s. Capacity Cost.}
When the compute resources are predefined, like in fixed-size virtual machines or containers, the total resources requirement for a shared-nothing distributed storage system is determined by the more restrictive of two factors: the performance limit or the storage capacity limit of individual nodes. 
%In environments where the types of machines are fixed in the cloud environment, the total resources required for a shared-nothing distributed storage system are determined by either the maximum performance of a single machine or its data storage capacity. This is because each machine operates independently, housing its own processor, memory, and storage. As such, the system's overall capability is constrained by the individual limits of these machines.

If the performance of a node, such as CPU speed, memory bandwidth, or disk IOPS, becomes the bottleneck, the system will need to scale out by adding more nodes to meet the performance requirements. In this case, the performance cost will drive the overall cost of the system.
On the other hand, if the storage capacity of a node becomes the limiting factor, the system will need to scale out to accommodate the data storage requirements. In this scenario, the capacity cost will be the primary driver of the overall cost.

Therefore, the overall cost of the system will be driven by the higher of the two costs (performance or capacity), as the system needs to scale based on the more restrictive aspect to meet the desired performance and storage objectives.


%If the machine's performance—reflected in metrics like CPU speed, memory bandwidth, and disk IOPS—is the limiting factor, then the performance cost will drive the total cost. This is because the system would need more machines to compensate for any individual machine's performance limitations to meet the desired speed and efficiency.

%On the other hand, if the data storage capacity of a machine is the bottleneck—due to the physical size of memory or disk space, then the capacity cost becomes the determining factor. In-memory systems, where memory is a premium resource, are particularly susceptible to this, as the cost of RAM significantly impacts the overall storage cost.

In Figure \ref{fig:cost-model}, we illustrate both the performance and storage costs. For workloads where the performance cost exceeds the storage cost, we categorize them as performance-critical workloads. Conversely, when the storage cost is dominant, we refer to these as storage-critical workloads.




\subsection{The Simplified Cost Model}
\label{The Simplified Cost Model}
Based on the above observations, we propose the following simplified cost model to quantify the cost for given key-value workload on specific shared-nothing storage system. Note that it assumes a homogeneous request profile and averages over the workload, similar to the Five-Minute Rule \cite{gray19875}.

Given a dataset $D$ and an access distribution, we define two key cost metrics in the model as follows:
\begin{definition}[Performance Cost per Query per Second ($CostPerQPS$)] 
$CostPerQPS$ is the average cost incurred for processing each request per second.
\end{definition}
\begin{definition}[Capacity Cost per GB ($CostPerGB$)] %\vspace{-1ex}
$CostPerGB$ is the cost for storing each gigabyte of data.
\end{definition}
The performance cost is calculated as $CostPerQPS \times QPS$, and the capacity cost is $CostPerGB \times Capacity$. The overall $Cost$ of the storage system is represented by the following equation:
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{5pt}
\begin{align}
Cost = \max (CostPerQPS \times QPS, CostPerGB \times Capacity )
\end{align}

The rationale behind using the maximum function is to capture the scenario where either the performance or capacity cost dominates, depending on the system's operational constraints or optimization objectives. This approach is particularly relevant in environments where ensuring performance SLAs or minimizing storage costs takes precedence.

For a tiered storage system, the total cost should include the cost of both cache(in-memory) tier and storage tier; thus, their cost model can be indicated as below 
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{5pt}
\begin{align}
Cost_{tiered} = \max(& CostPerQPS_{cache} \times QPS, \nonumber \\
                     & CostPerGB_{cache} \times Capacity \times \alpha) \nonumber \\
                 + \max(& CostPerQPS_{storage} \times QPS \times \beta, \nonumber \\
                     & CostPerGB_{storage} \times Capacity)
\end{align}
where $\alpha$ is the ratio of the storage capacity between fast tier and storage tier. $\beta$ is the general cache missing rate for accessing of the storage tier.

Please note that the cost model assumes an average record size for the workload. While this simplification may not capture all variations in record sizes, it provides a practical approximation for cost analysis.

\subsection{The Strategy to Minimize Cost}
\label{interval}

This subsection propose a strategy to minimize $Cost$ of two different single-tier storage systems. We revisit the concept of the Five-Minute Rule \cite{gray19875,five20,five30} as originally introduced, reformulating it to suit our context. The Break-Even Interval, a crucial metric in this rule, is defined by the following equation:
{\small
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{5pt}
\begin{align}
BreakEvenInterval &= \left( \frac{PagesPerMBofRAM}{AccessPerSecondPerDisk} \right) \nonumber \\
&\quad \times \left( \frac{PricePerDiskDrive}{PricePerMBofRAM} \right) \label{eq:rule_equation}
\end{align}
}

The Five-Minute Rule provides a framework for comparing the cost-effectiveness of two different storage media within a database system. 
In the context of comparing two distinct single-tier storage systems, we can extend the idea to evaluate the trade-offs between a high-performance, high-cost storage (Fast Storage) and a more economical, lower-performance storage (Slow Storage).


%Since the storage with lower performance and higher capacity cost is not a viable option, we posit that for any pair of storage $A$ and storage $B$, the following inequality must be satisfied:
%{\small
%\begin{align}
%    (CostPerGB_{A} - CostPerGB_{B} )  \nonumber \\
%    \times (CostPerQPS_{A} - CostPerQPS_{B}) < 0
%\end{align}
%}


\begin{definition}[Fast Storage] 
This storage type prioritizes performance and offers low latency and high throughput. It typically has a higher cost per GB ({\small$CostPerGB_{fast}$}) but a lower cost per query per second ({\small$CostPerQPS_{fast}$}).
\end{definition}

\begin{definition}[Slow Storage]
This storage type prioritizes capacity and cost-effectiveness over performance. It typically has a lower cost per GB ({\small$CostPerGB_{slow}$}) but a higher cost per query per second ({\small$CostPerQPS_{slow}$}).
\end{definition}
In comparison to HBase \cite{hadoop}, Redis \cite{redis} is commonly perceived as a Fast Storage due to its reliance on in-memory data storage. Similarly, the activation of data compression mechanisms can reduce the storage overhead, but this comes with a trade-off in terms of performance degradation. Hence, a database utilizing compression is deemed to be a Slow Storage when compared to one without compression.

The equilibrium point to minimize $Cost$ is derived from the interplay of their performance and capacity costs:
{\small
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{5pt}
\begin{align}
CostPerQPS_{slow} \times QPS &= CostPerGB_{fast} \times Capacity \label{eq:cache_cost} 
\end{align}
}

Subsequently, we can determine the break-even interval  associated with the minimization of $Cost$.
{\small
\begin{align}
BreakEvenInterval &= \frac{RecordNum}{QPS} \label{eq:def_break} \\
&= \frac{Capacity}{QPS\times AverageRecordSize} \label{eq:infer_break} \\
&= \frac{CostPerQPS_{slow}}{CostPerGB_{fast} \times AverageRecordSize} \label{eq:break_even_interval}
\end{align}
}
where Equation \ref{eq:infer_break} can be derived from Equation \ref{eq:def_break} due to $Capacity = RecordNum \times AverageRecordSize$.
% \begin{align}
% CostPerQPS_{slow} \times QPS &= CostPerGB_{fast} \times Capacity \label{eq:cache_cost} 
% \end{align}

In the context of the original Five-Minute Rule:
\begin{itemize}%[leftmargin=*]
    \item The ratio $\left( \frac{PricePerDiskDrive}{AccessPerSecondPerDisk} \right)$ effectively represents the $CostPerQPS_{slow}$.
    \item $PricePerMBofRAM$ correlates to $CostPerGB_{fast}$.
    \item $PagesPerMBofRAM$ is conceptually similar to $\left( \frac{1GB}{AverageRecordSize} \right)$.
\end{itemize}

The break-even interval analysis provides a critical strategy for optimizing storage system design. When the access interval of the data is shorter than the break-even interval, employing fast storage is advantageous due to its performance benefits. Conversely, when the access interval exceeds the break-even interval, utilizing slower storage is more cost-effective, as it optimizes for capacity.

This refined interpretation aligns with the original premise of the Five-Minute Rule, adapting it to our model's framework to evaluate the efficiency of storage systems in a modern context.
Moreover, utilizing the aforementioned model, we can calculate the break-even interval that compares tiered storage with single-tier storage systems, thereby extending the principles of the Five-Minute Rule. 

Our comprehensive experiments rigorously assessed the performance and cost efficiency of our system against leading open-source key-value databases using the introduced cost model. The evaluation results on real application workloads demonstrate the cost model's effectiveness in guiding cost-saving database system designs. 
Furthermore, the case study in Section \ref{case_study} showcases how the break-even interval helps choose the most cost-effective TierBase configuration.

A more comprehensive cost model analysis, including a comparison of costs between single-tier and disaggregated cache-storage architectures, is left for future work due to space constraints.
%The findings from our study can be used as standards for future work in creating more cost-effective storage options, showing that our cost model works well in actual situations.





